Diagnosing Medical Datasets with Training Dynamics

This study explores the potential of using training dynamics as an automated alternative to human annotation for evaluating the quality of training data. The framework used is Data Maps, which classifies data points into categories such as easy-to-learn, hard-to-learn, and ambiguous (Swayamdipta et al., 2020). Swayamdipta et al. (2020) highlight that difficult-to-learn examples often contain errors, and ambiguous cases significantly impact model training. To confirm the reliability of these findings, we replicated the experiments using a challenging dataset, with a focus on medical question answering. In addition to text comprehension, this field requires the acquisition of detailed medical knowledge, which further complicates the task. A comprehensive evaluation was conducted to assess the feasibility and transferability of the Data Maps framework to the medical domain. The evaluation indicates that the framework is unsuitable for addressing datasets' unique challenges in answering medical questions.

==> Figures/table-instance.tex <==
\begin{table*}[t!]
    \centering
    \caption{}
    \begin{tabularx}{\linewidth}{@{}lL{6cm}>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X@{}}
        \toprule
        & Instance & A & B & C & D \\
        \midrule
        \addlinespace[0.5em] % Add vertical space (adjust the value as needed)
        \multirow{2}{*}{\rotatebox{90}{\textit{easy-to-learn}}} 
            & Drug of choice for Herpes simplex encephalitis is: & 5-Hydroxy deoxyuridine (5-HU) &Acyclovir & Gancyclovir& None of the above \\
            & Schizophrenia is treated by: & Anti depressants &Anti psychotics&Anti epileptics& Mood stabilizers\\
        \multirow{2}{*}{\rotatebox{90}{\textit{hard-to-learn}}} 
            & Heparin is the commonly used anticoagulant in cardiac surgery. All of the following are true about heparin except: & Weakest acid found in living things &Most commercial preparations of heparin now utilize pig intestinal slimes & Act via Antithrombin activation& Produce thrombocytopenia \\
            & Schizophrenia is treated by: & Anti depressants &Anti psychotics&Anti epileptics& Mood stabilizers\\
        \multirow{2}{*}{\rotatebox{90}{\textit{ambiguous}}} 
            & Drug of choice for Herpes simplex encephalitis is: & 5-Hydroxy deoxyuridine (5-HU) &Acyclovir & Gancyclovir& None of the above \\
            & Schizophrenia is treated by: & Anti depressants &Anti psychotics&Anti epileptics& Mood stabilizers\\
        \addlinespace[0.5em] % Add vertical space (adjust the value as needed)
              \bottomrule
    \end{tabularx}
    \label{table:results}
\end{table*}
